On Transportability for Structural Causal Bandits

Intelligent agents equipped with causal knowledge can optimize their action spaces to avoid unnecessary exploration. The structural causal bandit framework provides a graphical characterization for identifying actions that are unable to maximize rewards by leveraging prior knowledge of the underlying causal structure. While such knowledge enables an agent to estimate the expected rewards of certain actions based on others in online interactions, there has been little guidance on how to transfer information inferred from arbitrary combinations of datasets collected under different conditions -- observational or experimental -- and from heterogeneous environments. In this paper, we investigate the structural causal bandit with transportability, where priors from the source environments are fused to enhance learning in the deployment setting. We demonstrate that it is possible to exploit invariances across environments to consistently improve learning. The resulting bandit algorithm achieves a sub-linear regret bound with an explicit dependence on informativeness of prior data, and it may outperform standard bandit approaches that rely solely on online learning.

==> Materials/algorithm_bandit.tex <==
\begin{algorithm}[t]
\small
% \SetAlgoNoEnd
% \SetAlgoVlined
\DontPrintSemicolon
\SetKwInput{KwInput}{Input}
% \SetKwInput{KwOutput}{Output}
\KwInput{Causal diagram $\mc{G}$, reward variable $Y$, non-maipulable variables $\mf{N}$, trials $T$, tolerance $\delta \in (0,1)$.}
% \KwOutput{Partial Topological Order over $\mc{P}[\mf{A}]$}

\setcounter{AlgoLine}{0}
\BlankLine 

$\mb{P}_{\mc{G,}Y}^{\mf{N}} = \textsf{POMISs}(\mc{G},Y,\mf{N})$; $\mc{I}_{\mc{G},Y}^{\mf{N}} = \{\mf{x} \in \Omega_{\mf{X}} \mid \mf{X} \in \mb{P}_{\mc{G},Y}^{\mf{N}}\}$ \;

Parameterize canonical representations of the quantities $Q[\mf{C}]$ for $\mf{C} \in \mb{C}_{\mc{G,}Y}^{\mf{N}}$ with $\omega = (\theta,\xi)$ based on $\mc{G}$.\;

% Choose each arm $\mf{x} \in \mc{I}_{\mc{G},Y}^{\mf{N}}$ once.\;

\While{\rm $\mc{L}_2$ exploration}
    {
    Intervenes on $\mf{x}_t \in \mc{I}_{\mc{G},Y}^{\mf{N}}$.
    }
% all trial $t=\vert \mc{I}_{\mc{G},Y}^{\mf{N}} \vert+1,\cdots, T$
\For{\rm all trials $t \leq T$}{
    \ding{172} For all $\mf{x} \in \mc{I}_{\mc{G},Y}^{\mf{N}}$, update estimated interventional probability $\hat{P}_\mf{x}$.  
    % For every $\mf{C} \in \mb{C}_{\mc{G,}Y}^{\mf{N}}$, update $\hat{Q}_t[\mf{C}] = [P_{\mf{x},t}]_{w}$.\;

    \ding{173} Set confidence set $\mb{M}_t$ which consists of canonical SCMs with respect to $\omega = (\theta, \xi)$ satisfying that for every $\mf{x} \in \mc{I}_{\mc{G},Y}^{\mf{N}}$
    \setlength{\belowdisplayskip}{0pt}%
    \setlength{\abovedisplayskip}{0pt}%  
    \begin{align}
        \lVert P_\omega - \hat{P} \Vert_{1} \leq  \sqrt{\frac{?}{?}}
    \end{align}

    \ding{174} Find the optimistic arm $\mf{x}_t$ such that\;
    \setlength{\belowdisplayskip}{0pt}%
    \setlength{\abovedisplayskip}{0pt}%  
    \begin{align}
        \mf{x}_t =
        \underset{\mf{x} \in \mc{I}_{\mc{G},Y}^{\mf{N}}}{\mathrm{argmax}}\max_{\mc{M} \in \mb{M}_t} \mu_\mf{x}
    \end{align} and intervenes on $\mf{x}_t \in \mc{I}_{\mc{G},Y}^{\mf{N}}$.
    
}%end For
\caption{Info Sharing Causal-UCB (\textsf{ISC-UCB})}
\label{alg: bandit}
\end{algorithm}


